BFRT: Blockchained Federated Learning for Real-time Traffic Flow Prediction

Accurate real-time traffic flow prediction can be leveraged to relieve traffic congestion and associated negative impacts. The existing centralized deep learning methodologies have demonstrated high prediction accuracy, but suffer from privacy concerns due to the sensitive nature of transportation data. Moreover, the emerging literature on traffic prediction by distributed learning approaches, including federated learning, primarily focuses on offline learning. This paper proposes BFRT, a blockchained federated learning architecture for online traffic flow prediction using real-time data and edge computing. The proposed approach provides privacy for the underlying data, while enabling decentralized model training in real-time at the Internet of Vehicles edge. We federate GRU and LSTM models and conduct extensive experiments with dynamically collected arterial traffic data shards. We prototype the proposed permissioned blockchain network on Hyperledger Fabric and perform extensive tests using virtual machines to simulate the edge nodes. Experimental results outperform the centralized models, highlighting the feasibility of our approach for facilitating privacy-preserving and decentralized real-time traffic flow prediction.

==> 3-Problem_Description.tex <==

\section{Problem Description}
% Here we want to define the problem mathematically. We have a set of deployed traffic collection devices and RSUs deployed at the netwotk edge which independently collect local traffic data within their vicinity. These devices are owned by a set of one or more participating organizations, who seek to collaboratively train an adaptable and online model without exposing or sharing their underlying sensitive data. 

% Within the scope of this work, we define the FL traffic flow prediction problem as an arterial corridor prediction problem. Within the corridor, we have a set of one or more organizations representing company-based entities. Each organization manages and operates a set of deployed traffic collection edge devices $E = \{e_1, e_2, ..., e_n\}$ along the corridor. These devices can represent CAVs, RSUs, base stations, and any other deployed IoV device facilitating the collection and processing of traffic flow data. In our case study, the organizations seek to cooperatively train an online and dynamic prediction model leveraging their collected traffic data in real-time, while ensuring data privacy is preserved and without the need to share the underlying data between participants. Additionally, the organizations wish to avoid the need to transmit large amounts of collected data to a centralized data center or cloud for processing, and wish to perform computations and model training directly on deployed devices at the IoV network edge. 

% In alignment with the design framework of Hyperledger Fabric, we also define the following additional entities within the context of the blockchain network: clients, peers, and orderers. The set of clients $C = \{c_1, c_2, ..., c_n\}$ are the network participants who can interact with the blockchain and smart contracts, but do not expend additional computation resources on blockchain management operations (e.g., storage, validation, consensus). In our design, clients are a subset of traffic collection edge devices who collect local traffic data and train localized prediction models, and seek to participate in the FL process. Peers $P = \{p_1, p_2, ..., p_n\}$ represent the blockchain participants who perform transaction validation and storage functions through maintaining a copy of the blockchain ledger. They are also a subset of the traffic collection edge devices, and are generally deployed alongside the data collectors to alleviate the computational burden of blockchain management from the collectors. Lastly, orderers $O = \{o_1, o_2, ..., o_n\}$ are the blockchain nodes tasked with consensus processing who order the transactions and group them into blocks, ensuring fault tolerance for the network. These devices are owned and operated by the organizations, and can have more deployment flexibility. Generally, these devices can either be powerful servers which reside further inside the network at data centers/cloud, or can be deployed at the network edge in a containerized fashion on the same low-powered devices which operate the blockchain peers. Notably, the deployment strategy for orderers can significantly impact the network performance. 


Within the scope of this work, we define the FL traffic flow prediction problem as an arterial corridor prediction problem. Within the corridor, we have a consortium of one or more organizations representing company-based entities (e.g., DoT, Uber, Doordash). Each organization manages and operates a set of deployed RSUs, which act as traffic collection edge devices, along the corridor. In our case study, the organizations seek to cooperatively train an online and dynamic prediction model leveraging their collected traffic data in real-time, while ensuring data privacy is preserved and without the need to share the underlying data between participants. Additionally, the organizations wish to avoid the need to transmit large amounts of collected data to a centralized data center or cloud for processing, and wish to perform computations and model training directly on deployed devices at the IoV network edge. Moreover, the RSU devices are already computationally-burdened with data collection and model training operations, and the organizations desire for the parameter server operations to be offloaded to nearby edge devices dedicated to this task. 

In alignment with the design framework of Hyperledger Fabric, we define the following entities within the context of our proposed system architecture and map them to the participating devices: clients, peers and orderers. The set of clients $C = \{c_1, c_2, ..., c_n\}$ are the network participants who can interact with the blockchain, 
%and smart contracts,
but do not expend additional computation resources on blockchain management operations (e.g., storage, validation, consensus). In our design, clients represent the RSU devices who collect local traffic data, train localized prediction models, and also participate in the FL process. Peers $P = \{p_1, p_2, ..., p_n\}$ represent the blockchain participants who perform transaction validation and storage functions through maintaining a copy of the blockchain ledger. In our architecture, the peers represent lightweight IoV edge devices (e.g., Raspberry Pi), and are generally deployed alongside the data collectors to alleviate the computational burden of blockchain management from the RSUs. Lastly, orderers $O = \{o_1, o_2, ..., o_n\}$ are the blockchain nodes tasked with consensus processing who order the transactions and group them into blocks, ensuring fault tolerance for the network. These devices are owned and operated by the organizations, and can have more deployment flexibility. Generally, these devices can be more powerful base stations or mobile edge computing servers, capable of processing large transaction loads and supporting the FL process. Notably, the deployment strategy for orderers can significantly impact the network performance. 



